Asteria-Pro: Enhancing Deep-Learning Based Binary Code Similarity Detection by Incorporating Domain Knowledge

The widespread code reuse allows vulnerabilities to proliferate among a vast variety of firmware. There is an urgent need to detect these vulnerable code effectively and efficiently. By measuring code similarities, AI-based binary code similarity detection is applied to detecting vulnerable code at scale. Existing studies have proposed various function features to capture the commonality for similarity detection. Nevertheless, the significant code syntactic variability induced by the diversity of IoT hardware architectures diminishes the accuracy of binary code similarity detection. In our earlier study and the tool Asteria, we adopt a Tree-LSTM network to summarize function semantics as function commonality and the evaluation result indicates an advanced performance. However, it still has utility concerns due to excessive time costs and inadequate precision while searching for large-scale firmware bugs. To this end, we propose a novel deep learning enhancement architecture by incorporating domain knowledge-based pre-filtration and re-ranking modules, and we develop a prototype based on Asteria called Asteria-Pro. Pre-filtration module seeks to eliminates dissimilar functions to boost subsequent deep learning model calculations, while re-ranking module aims to raises the rankings of vulnerable functions among candidates generated by deep learning model. Our evaluation indicates that pre-filtration module cuts the calculation time by 96.9% and re-ranking improves MRR and Recall by 23.71% and 36.4%. By incorporating the pre-filtration and re-ranking modules, Asteria-Pro outperforms existing state-of-the-art approaches in bug search task, by a significant large margin. We conduct a large-scale real-world firmware bug search and Asteria-Pro manages to detect 1,482 vulnerable functions with a high precision 91.65%.

==> filtration.tex <==
\section{DK-based Prefiltration} \label{sec:prefiltration}

At this stage, \toolname{} intends to incorporate a efficient and effective filter.
To this end, we propose three requirements (\cref{sec:requirements}) to guide feature selection for constructing such filter.
To evaluate the features, we prepare code base and introduce various metrics (\cref{sec:benchmark}).
To find suitable features, we first choose popular traditional features applied by many works for evaluation and comparison (\cref{sec:feature_eval}).
We propose a new feature and a new algorithm to construct our intended filter based on the evaluation results and bad case analysis(\cref{sec:new_feature}).


\subsection{Filter Requirements} ~\label{sec:requirements}
The efficiency of filter requires it to remove as many non-homologous functions as possible in a very short time.
The effectiveness of filter requires it to preserve all homologous functions.
%The lightweight seeks simple but \textbf{robust syntactic features}, where robustness means features do not change over different compilation settings.
We summary the filter requirements as follows:
\begin{itemize}
    \item [R1.] \textit{The filter retains all homologous functions (i.e., extreme high true positive rate).} This requirement ensures that in filter phase, we do not miss any homologous functions.
    \item [R2.] \textit{The filter removes as many non-homologous functions as possible (i.e., low false positive rate).} This requirement ensures that the number of non-homologous functions going to the next round of model computations is as small as possible.
    \item [R3.] \textit{The filter performs very fast calculations.} This requirement ensures the filtration overhead time is as short as possible. %than time for next computation.
\end{itemize}


\subsection{Evaluation Benchmark} \label{sec:benchmark}
\subsubsection{Code Base} \label{sec:codebase}
%compilation
To derive robust features, we compile a large collection of binaries from 184 open source software (OSS), such as OpenSSL, FFmpeg, Binutils, etc.
Since our tool aims to detect homologous functions across different architectures, we compile these OSS to 4 different architectures, X86, X64, ARM, and PowerPC.
Besides, we take the default compilation settings during compilation to be in line with the real situation use.
After compilation, there are many test binaries generated with ``test'' or ``buildtest'' as a prefix or suffix, to test functionality of the software.
We remove these test binaries from the collection since the functions in these binaries, 1) are simple and only consist of several lines of code. 2) are not involved in the real execution of software function.
After removal, a total of 1130 binaries, 226 for each architecture, are retained in binary collection.

% dataset construction.
We construct a large groundtruth dataset containing homologous functions and non-homologous functions.
To this end, we keep the function names during the compilation.
We use binary functions with the same function name in the same software to form homologous functions, otherwise they form non-homologous functions.
For example, supposing function $F$ is present in the source code, compilation will results in 5 versions of binary functions for different instruction set architectures: $F_{x86}$, $F_{x64}$, $F_{arm}$, $F_{ppc}$, and $F_{mips}$ respectively.   
Then we have $F_{x86}$, $F_{x64}$, $F_{arm}$, $F_{ppc}$, and $F_{mips}$, which are homologous functions of each other.
For other binary function $f_{arch}$ ($arch$ could be x86, x64, arm, ppc, mips), we say that $f_{arch}$ are non-homologous function of any of $F_{x86}$, $F_{x64}$, $F_{arm}$, $F_{ppc}$, and $F_{mips}$.
% function pairs
We extract 53,516 unique binary functions for each architecture, for a total of 267,580 binary functions.
We split the code base into two datasets:
\begin{itemize}
    \item \textbf{Prefiltering dataset.} We choose 10,000 functions at random from a pool of 53,516 to assess the robustness of various features and test the ability of the filter.
    \item \textbf{Training dataset.} The left functions will be used to train and test Tree-LSTM models,
    \item \textbf{Evaluation dataset.} We choose xxx function at random from left functions for function similarity detection methods. 
\end{itemize}

\subsubsection{Metrics} \label{sec:metrics}
%First, we describe the details of metrics calculation of recall and false positive rate.
We use two metrics to evaluate the filtering ability of different features: true positive rate (TPR) and false positive rate (FPR).
TPR shows the feature ability to retrieve homologous functions and FPR shows the ability to filter out non-homologous functions.
In the filtering stage, our principle is \textit{to use features that can filter out non-homologous functions as much as possible (low FPR) on the basis that all homologous functions can be retained (very high TPR)}.

We prepare the homologous function pairs and groups for feature evaluations.
Specifically, we utilize the source function name $F$ together with the library name $B$, since function names in different binaries might be duplicated but having different functionalities, to combine into a function identifier $F^{B}$.
After compilation, we will get different homologous binary functions for different architectures, X86 ($F^{B}_{X86}$), X64 ($F^{B}_{X64}$), ARM ($F^{B}_{ARM}$), MIPS ($F^{B}_{MIPS}$), PowerPC ($F^{B}_{PPC}$).
These five binary versions of function form a homologous function groups.
We pick a random version of function to combine with other 4 versions of functions to form 4 homologous function pairs.
We calculate different metrics for function pairs and groups respectively.

Suppose we select $N$ functions from all $M$ functions as `hypothetical vulnerable functions`, we first pick a random version of `vulnerable` function $F^{B}_{X}$, since the vulnerable function could be from any architecture. 
Then we calculate the feature scores between $F^{B}_{X}$ and other $M \times 5 - 1$ binary functions, where 5 means the number of architectures.
As a result, $M \times 5 - 1$ function pairs consist of $4$ homologous pairs and $M \times 5 - 5$ non-homologous pairs.
Then we filter out function pairs whose scores are less than a threshold value $T$.
%After the filtering, we adopt two different evaluation granularities, pair metric and group metric, to assess the quality of features.
%In pair metric, in the function pair after filtering,
After the filtering, in the resulting function pairs, the homologous function pair is regarded as a true positive $TP$, and a non-homologous function pair is regarded as a false positive $FP$.
To assess the ability cross all architectures, we also adopt a more strict metric $TP^{2}$, in which only if all homologous pairs are preserved, the filtering result is regarded as a true positive.

We calculate these three metrics for different features as shown in following equations:
\begin{gather} \label{eq:recall_fp}
	TPR = \frac{\sum_{i=1}^nTP_i^p}{4 \times n} \\ 
    recall = \frac{TP^2}{n} \\
    FPR =  \frac{\sum_{i=1}^nFP_i}{n \times (M \times 5-5)}
\end{gather}
In the equation, `$M \times 5 - 5$' means the number of homologous functions of one target function.


% how to write the story to compare with other method?
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{pics/source_to_ast.pdf}
    \caption{AST Example}
    \label{fig:ast}
\end{figure}

\subsection{Traditional Features Evaluation} \label{sec:feature_eval} 
%To identify robust syntactic features, We evaluate \todo{xx} features on the \textbf{prefiltering dataset}: string literal, callee functions, AST size.
We aim to discover the features that satisfy our filter requirements to integrate in filter.
First, we tend to evaluate features proposed in previous works.
Based on the evaluation results, we select and improve the features that are candidates for the filter requirements.
%and find that the feature related to function call relation performs better.
%To fully exploit the information from call relation, we design a new feature and a new algorithm for it.
% only number, not semantic infos
%However, these works only consider the statistic feature of call relationship, not fully exploit it.






\noindent
\textbf{Feature Description.}
Many tradition features are proposed in previous works \todo{CITATION} to apply to homologous binary function detection.
Considering the filter requirement R3, we intend to chose lightweight and robust features.
We divide tradition features into two categories: CFG-family feature and AST-family feature.
CFG-family features include 5 numeric features: \textit{the number of instructions, arithmetic instructions, call instructions, logical instructions, transfer instructions}, and 2 constant features: \textit{string constants and numeric constants}~\todo{CITATION DiscovRE}.
To evaluate the features, DiscovRE, which is the first to present these features, considers the correlation of features to ensure the recall rate of homologous functions. 
However, such evaluation in DiscovRE does not indicate the requirements introduced in \cref{sec:requirements}.
Since the first two requirements R1 and R2 can be indicated by true positive rate and false positive rate separately, we evaluate the filtering ability of these features using these two metrics.

In addition to features proposed from DiscovRE, we also define several syntactic features as AST-family features as following:
\begin{itemize}
    \item No. AST Nodes. The number of AST nodes.
    \item AST node Cluster. The number of different node types in AST.  For example, in Figure~\ref{fig:ast}, the AST node Cluster is denoted as $[block: 3, if: 1, return: 1, call: 1, num: 3, block: 2, asg: 2, var: 4, le: 1]$
    \item AST Fuzzy Hash. We first generate node sequence by  traversing the AST preorder. Then we apply the fuzzy hash algorithm~\todo{CITATION} to generate the fuzzy hash of AST.
\end{itemize}

\todo{The reasons to define above features.}



\noindent
\textbf{Feature Similarity Calculation.}
Features are classified into two types for similarity calculation: value type and sequence type.
Value type features consist of \textit{No. Instruction}, \textit{No. Arithmetic}, \textit{No. Logic}, \textit{No. Callee}, and \textit{No. AST nodes}.
Sequence type features consist of \textit{Numeric Constant}, \textit{String Constant}, \textit{AST Node Cluster}, and \textit{AST Seq Hash}.
For value type features, we use the relative difference ratio ($RDR$) as shown below for similarity calculation:
\begin{equation}\label{eq:rdr}
    RDR(V_1, V_2) = 1-\frac{ abs( V_1 - V_2)}{max(V_1, V_2)}
\end{equation}
\noindent where $V_1, V_2$ are feature values.

For each sequence type feature, we first sort the elements of feature and concatenate them as an unified sequence.
Then we use the common sequence ratio ($CSR$) based on longest common sequence (LCS) as following:
\begin{equation}\label{eq:csr}
    CSR(S_1, S_2) = \frac{2 \times LCS( S_1, S_2)}{len(S_1) + len(S_2)}
\end{equation}
where $S_1, S_2$ are feature sequences, and function $LCS(\cdot, \cdot)$ returns the length of the longest common sequence between $S_1, S_2$.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{pics/roc_old_fea.pdf}
    \caption{ROC Curves for Traditional Features.}
    \label{fig:roc_old_fea}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{pics/filter_time_cost.pdf}
    \caption{Time Costs of Similarity Calculation for Different Features.}
    \label{fig:fea_time_cost}
\end{figure}

\noindent
\textbf{Evaluation Results.}
We calculate the FPRs and TPRs for each feature using various similarity thresholds and plot them as receiver operating characteristic (ROC) \todo{CITATION} curve, as shown in Figure~\ref{fig:roc_old_fea}.
%The evaluation results are shown in Figure~\ref{fig:roc_old_fea}.
We also calculate the area under ROC curve (AUC), which indicates how well the feature can separate homologous and non-homologous functions.
As shown in figure, the features extracted from AST (i.e., \textit{No. AST Nodes}, \textit{AST Node Cluster}, and \textit{AST Seq Fuzzy Hash}) have high AUC values.
However, they are unable to meet both R1 and R2.
In other words, they generate a sizably FPR under high TPR.

Furthermore, we plot the time costs of similarity calculations for different features as shown in Figure~\ref{fig:fea_time_cost}.
As we can see, sequence type features take longer than value type features.
Nevertheless, the order of magnitude of their time consumption is within an acceptable range.
To be precise, at least $10^5$ calculations can be performed per second.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{pics/fscore_old_fea.pdf}
    \caption{$F_{score}$ of Traditional Features.}
    \label{fig:fscore_old_fea}
\end{figure}

We notice that in Figure~\ref{fig:roc_old_fea}, under high TPR (0.996), the feature \textit{No. Callee} produces relatively lower FPR (0.111).
Recalling our goal in the filtering phase, we aim to select features with a low FPR at a very high TPR. 
Features with high AUC do not necessarily meet the filtering requirements R1 and R2.
For example, the feature \textit{AST Node Cluster} has a higher FPR (0.47) than feature \textit{No. Callee} (FPR = 0.111) under the same TPR (0.996), even feature \textit{AST Node Cluster} has higher AUC (0.978) than feature \textit{No. Callee} (AUC = 0.944).
To this end, we propose a new metric $F_{score}$ to meet both R1 and R2.
\begin{equation}
    F_{score} = \frac{1}{\frac{1}{TPR} + FPR}
    \label{eq:fscore}
\end{equation}
\noindent For each feature, we calculate the $F_{score}$ and plot the $F_{score}$ curves in Figure~\ref{fig:fscore_old_fea}.
The Figure~\ref{fig:fscore_old_fea} plots $F_{score}$ curves of various features at various similarity thresholds.
The tuple in legend shows the feature name and the best $F_{score}$ at corresponding threshold (denoted as best=(threshold, $F_{score}$)) .
We can see that the feature \textit{No. callee} has the best $F_{score}$ (0.90) at threshold 0.94. 

Note that the feature \textit{No. callee} count only the number of callee functions, and excludes important information such as function names.
Feature \textit{No. callee} has room for further exploration.

To fully exploit the feature \textit{No. callee}, we manually analyze the incorrect results (i.e., false positives and false negatives) and summarize the challenges in order to fully utilize it:

\begin{itemize}
    \item \textbf{Exploitation Challenge 1 (EC1).} The name of callee function may be deleted. For safety and size reasons, the binary usually is stripped after compilation~\todo{CITATION}.
    The function names in the static symbol table are removed after strip.
    Such function names can not help exploit the function call relations.
    
    \item \textbf{Exploitation Challenge 2 (EC2).} There is no callee functions in some functions (i.e., leaf node in call graph).
    
    \item \textbf{Exploitation Challenge 3 (EC3).} Function calls in binary target functions might not always be consistent with source code. Function calls may be added or deleted due to compiler optimization.
    The reasons for the function call change are function inline, intrinsic function replacement, instruction replacement for optimization, that behave differently in different architectures. We describe this challenge in detail in \textbf{Function Call Optimization}.
   
    \item \textbf{Exploitation Challenge 4 (EC4).} There are several ways to decorate function names by compiler. The function name will differ from its original name in the source code after decoration.
    
    
\end{itemize}

For \textbf{EC4}, there are mainly two kinds of decoration ways: incremental modifications and function Replacement.

\noindent \textbf{Function Call Optimization.} 
The first optimization strategy is function inline, which is adopted in all kinds of compilers.
As mentioned in paper Asteria~\todo{CITATION}, function may be inline as a result of compilation optimization.
Bingo~\todo{CITATION} propose a selective inline algorithm to lessen the inline effects.
However, we are unable to afford such a costly algorithm that requires millisecond filtration.
The second optimization strategy is intrinsic function implementation, which is different in different instruction set compiler.
For example, the ARM compiler (gcc) has dedicated instructions for intrinsic functions (a.k.a. built-in functions) \todo{CITATION}.
As shown in Figure xxx.

\begin{minipage}[t]{\linewidth}
\centering
    \begin{minipage}[t]{\linewidth}
    \begin{lstlisting}
    unsigned int mysqrt(unsigned int x) {
        return sqrt(x);
    }
    \end{lstlisting}
    \captionof{figure}{Example Source Code}
    \end{minipage}

\begin{minipage}[t]{0.48\linewidth}
\begin{lstlisting}
mysqrt(ARM):
    vmov          s0, r0   
    vcvt.f64.u32  d16, s0   
    vsqrt.f64     d16, d16
    vcvt.u32.f64  s0, d16
    vmov          r0, s0
    bx            lr
\end{lstlisting}
\end{minipage}
\hspace{1pt}
\begin{minipage}[t]{0.5\linewidth}
\begin{lstlisting}
mysqrt(X86):
    subq    $24, %rsp
    movsd   %xmm1, 8(%rsp)
    call    sqrt@PLT
    movsd   8(%rsp), %xmm1
    addq    $24, %rsp
    cvttsd2siq      %xmm1, %rax
    ret
\end{lstlisting}
\end{minipage}
\caption{Intrinsic Function Example for ARM compared with X86.}
\end{minipage}

\todo{TODO.}


%1. 我们分析发现，1中提到的统计特征，在某些情况下是不适用的（产生FP、FN），但是callee 表现比较好。
%    a. callee_num 在旧特征中表现比较好。
%    i. 指令统计类特征，num constant特征一起AST seq size相关特征即便是最好情况下的tpr依然没能满足我们的要求（0.98以上），这可能会导致漏洞函数被漏报
%    ii. string特征有很好的tpr和fpr，但因为只有部分函数中存在，且占比较少，不能作为主要过滤特征
%    iii. 相比较而言，callee_num能够满足高tpr(0.99+)，过滤能力也比较高，但我们认为在fpr这块仍有改进空间（因为单单用num丢失了太多调用语义信息），所以我们针对callee这一特征进一步深入挖掘

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{pics/roc_new_fea.pdf}
    \caption{ROC Curves for New Features.}
    \label{fig:roc_new_fea}
\end{figure}
\subsection{Filter} \label{sec:new_feature}
To overcome exploitation challenges, we propose a new feature, named \textbf{genealogist} and a new algorithm, named \textbf{UpRelation} for exploiting the new feature.
\subsubsection{New Feature}
Our new feature intends to extract comprehensive information from the call relationship of the entire binary, including the symbol information.
Such call relationship can be denoted by \textit{call graph}.
The \textit{call graph} $CG$ can be defined by giving all functions as nodes and the call relationships between functions as edges: $CG = ( \mathcal{V},\mathcal{E} )$, where $\mathcal{V} = \{v| \text{$v$ is a function}\}$ denotes the node collection and $\mathcal{E} = \{ (u,v)| \text{$u$ calls $v$}\}$ denotes the edge collection.
For edge $(u,v) \in E$, we say that function $v$ is a callee function of function $u$.
%$CG = ( \{v| \text{$v$ is a function}\}, \{ (u,v)| \text{$u$ calls $v$}\})$.
The genealogist is a function list containing \textbf{partial} callee functions of the target function.
Considering \textbf{EC1}, we can not utilize all symbol information of callee functions, since callee functions might be in removable symbol table (i.e., static symbol table), and the function name will removed.
Fortunately, to link against dynamic libraries, function names in the dynamic symbol table $DST$ (i.e., import and export table) will be preserved \todo{CITATION}.
For example, if target function calls external function `strcpy', the callee function name `strcpy' remains in import table rather than removed after binary strip.
%, where function names keep the semantic information.
We define genealogist $GL$ of target function $f$ as: $GL_f = \{ v | v \in \mathcal{V}, (f, v) \in  \mathcal{E}, v \in DST \}$.%, where $callee_i$ denotes the name of callee function of $f$.
%Since the binary containing the target function usually be stripped, which means function names in the symbol table of binary are all deleted,

%To overcome \textbf{EC1}, we extract the callee function names that are recorded in import or export table to construct the $GL$.
Note that caller functions of target function are not considered in the $GL$, since the callers of target function may be inconsistent due to open-source component reuse in different software.
For example, suppose there is a function $Fc$ in a open-source component, such component is integrated by software $A$, where $Fc$ is called by $Fa$ in $A$.
Similarly, the component can be integrated by software $B$ and $Fc$ is called by $Fb$ in $B$.
In the above situation, function $Fc$ has different caller functions.
For cases where a function calls the same function multiple times, we keep multiple identical function names.


\iffalse
\begin{table}[t]
    \centering
    \caption{Evaluation of Different Features.}
    \begin{tabular}{c|c|c|c|c}
        Feature Name & $TPR$ & $FPR$ & $FP^2R$  & Time ($10^{-7}$s) \\
        \hline
        No. Instructions & 0.xx & 0.xx & 0.xx & 0.xx  \\
        No. Arithmetic & 0.xx & 0.xx & 0.xx & 0.xx \\
        No. Logic & 0.xx & 0.xx & 0.xx & 0.xx  \\
        No. Transfer & 0.xx & 0.xx & 0.xx & 0.xx  \\
        Numeric Constant  & 0.xx & 0.xx & 0.xx & 0.xx \\
        String Constant & 0.xx & 0.xx & 0.xx & 0.xx  \\
        \hline
        No. AST nodes  & 0.xx & 0.xx & 0.xx & 0.xx  \\
        AST seq count & 0.xx & 0.xx & 0.xx & 0.xx \\
        AST seq fuzzy hash& 0.xx & 0.xx & 0.xx & 0.xx \\
        \hline
        No. Callee & 0.xx & 0.xx & 0.xx & 0.xx\\
        Callee Seq   & 0.xx & 0.xx & 0.xx & 0.xx \\
        Callee Seq LCS & 0.xx & 0.xx & 0.xx & 0.xx \\
    \end{tabular}
    \label{tab:my_label}
\end{table}
\fi




%So we draw a horizontal line at $TPR=0.99$ for feature selection.

% new metric



\subsubsection{Filtration algorithm} \label{sec:filtermethod}
%We select the top 3 best-performing features to build our filter, genealogist, strings, and number of callees.
%However, these 3 features can not make sure to be present in a random function, e.g., a function that does not call other functions and does not also reference a string.
To support our new feature, we propose a feature similarity algorithm, called \textbf{UpRelation}.
The algorithm utilizes context information in the call graph to overcome challenge  \textbf{EC2}, \textbf{EC3}.
Specifically, the algorithm utilizes parent nodes of leaf nodes in call graph to match leaf nodes to address the \textbf{EC2}.
In the algorithm, we adopt a drill down strategy, that combines three feature $GL$, \textit{No. Callee}, and \textit{String Constants}. \todo{REASON.}
The \textit{No. Callee} of function $f$ is denoted by $Callee_f$ and the \textit{String Constant} set of function $f$ is denoted by $StrCons_{f}$.

\begin{algorithm}
\caption{UpRelation}
    \label{alg:uprelaiton}
    \SetKwFunction{RDR}{RDR} 
    \SetKwFunction{CSR}{CSR} 
    \SetKwFunction{GetCallers}{GetCallers}
    \SetKwFunction{GetCallees}{GetCallees}
    \KwIn{Vulnerable Function $fv$, Target Function List $TFL$, Thresholds $T_{GL}, T_{callee}, T_{string}$}
    \KwOut{Vulnerable Candidate Function List $VFL$}
    
    $VFL \gets TFL$\;
    
    \uIf{$GL_{fv}$ is not null}{
        \For{$f \in TFL $}
        {   
            $s$ = \CSR{$GL_{fv}$, $GL_{f}$}\;
            \lIf{$s < T_{GL}$}{$VFL$.pop($f$)}
        }
    }
    \uElseIf{$ Callee_{fv} > 0$ }{
        \For{$f \in TFL $}{
            $s$ = \RDR{$Callee_{fv}$, $Callee_{f}$}\;
            \lIf{$s < T_{callee}$}{$VFL$.pop($f$)}
        }
    }
    \uElse{
        % 叶子函数识别
        $FL'$ = $\emptyset$\;
        \For{$fp \in $ \GetCallers{fv}}{
            % 基于叶子函数的caller生成候选函数列表
            \For{$fp' \in UpRelation(fp, VFL)$}{
                $FL'$.add(\GetCallees{$fp'$})\;
            }
        }
        $VFL$ = $FL'$\;
        }
        
    \eIf{$StrCons_{fv}$ is not null}{
    \For{$f \in VFL$}{
         $s$ = \CSR{$StrCons_{fv}$, $StrCons_{f}$}\;
          \lIf{$s < T_{string}$}{$VFL$.pop($f$)}
      }    
  }
\textbf{return $VFL$}\;

\end{algorithm}

Given a vulnerable function $f_v$, Algorithm~\ref{alg:uprelaiton} aims to identify  vulnerable candidate function list ($VFL$) from target function list $TFL$.
The algorithm obtain the list $VFL$ by filtering out the irrelevant functions (i.e., not vulnerable).
Code from line 2 to line 6 performs filtering when feature genealogist $GL_{fv}$ of $f_v$ is not empty.
Specifically, the algorithm calculates the $CSR$ of Equation~\ref{eq:csr} between $GL_{fv}$ and $GL_f$ of all candidate functions in line 4.
Then it filters out functions whose $CSR$ is less than a threshold $T_{GL}$.
Similarly, when callee number $Callee_{fv}$ of $fv$ is not 0, it filters out functions by calculating $RDR$ score from line 7 to line 11.
Line 12 to 19 makes up the most crucial portion of the algorithm, which matches the leaf functions to address \textbf{EC2}.
%The algorithm's most important section, which matches the leaf functions to address \textbf{EC2}, runs from line 12 to line 19.
All caller functions of $fv$ are first visited in this section of the algorithm at line 14.
It employs $UpRelation$ to discover all functions that are similar to caller function, $fp$.
For each similar function $fp'$, the algorithm regards all its callee functions as vulnerable candidate functions at line 16.
%In this section of algorithm, it first visits all caller functions of $fv$ at line 14.
%For each caller function $fp$, it uses $UpRelation$ to find all functions similar to $fp$.
We find the same leaf functions by locating the same caller functions because the caller functions of the same leaf functions are also the same.
However, this introduces some extraneous (leaf) functions, that share the same caller function but are not the same as the leaf function.
We utilize string similarity at line 22, to remove extraneous functions.
After filtering by callees and strings, the algorithm finally gets the expected vulnerable candidate function list $VFL$.



\iffalse
\begin{algorithm}
\caption{UpRelation}
    \label{alg:uprelaiton}
    \SetKwFunction{LCSScore}{LCSScore} 
    \SetKwFunction{NumericScore}{NumericScore} 
    \KwIn{Vulnerability function $f_v$, Candidate function list $L_f$}
    \KwOut{Filtered function list $L_f$}
    

    \For{$f \in L_f $}
    {   

        \eIf{$f_v.Genealogist.length > 0$}{
            $s$ = \LCSScore{$f_v.Genealogist$, $f.Genealogist$}\;
            \lIf{$s < threshold$}{$L_f$.pop($f$)}
          }{
            \eIf{$f_v.callee.length > 0$ }{
                $s$ = \NumericScore{$f_v.callee.length$, $f.callee.length$}\;
                \lIf{$s < threshold$}{$L_f$.pop($f$)}
            }{
            % 叶子函数识别
            $L_f'$ = $\emptyset$\;
            \For{$f_p \in f_v.caller$}{
                % 基于叶子函数的caller生成候选函数列表
                \For{$f_p' \in UpRelation(f_c, L_f)$}{
                    $L_f'$.add($f_p'.callee$)\;
                }
            }
            $L_f$ = $L_f'$\;
            }
        }
        \eIf{$f_v.strings.length > 0$}{
         $s$ = \LCSScore{$f_v.strings$, $f.strings$}\;
          \lIf{$s < threshold$}{$L_f$.pop($f$)}
          }{
          do nothing\;
      }     
    }
    \textbf{return $L_f$}
    
    

    
    
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\LCSScore{$seq_1$, $seq_2$}}{
        $$ score = \frac{2*\LCS(seq_1,seq_2).length}{seq_1.length + seq2.length}$$
       
        \textbf{return} $score$
    }
    
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\NumericScore{$num_1$, $num_2$}}{
        $$score = \frac{\min(num_1,num_2)}{\max(num_1, num_2)}$$
       
        \textbf{return} $score$
    }

    
\end{algorithm}
\fi

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{pics/fscore_new_fea.pdf}
    \caption{$F_{score}$ of new feature.}
    \label{fig:fscore_new_fea}
\end{figure}

\subsubsection{Filtration Method Evaluation}
We evaluate the variants of feature \textbf{genealogist} and the algorithm \textbf{UpRelation}.
The variants consist of plain \textbf{genealogist} (denoted as \textbf{Genealogist}), the LCS score of \textbf{genealogist} (denoted as \textbf{Genealogist LCS}).
The algorithm employs the \textbf{Genealogist LCS} and is denoted as \textbf{Genealogist LCS+UpRelation}.
To gain a more intuitive comparison with traditional features, we use the feature \textbf{No. Callee} as a baseline, which performs best among all traditional features.
We calculate the TPRs and FPRs under different thresholds for each features and use the receiver operating characteristic (ROC) curve to display the results.

As Figure~\ref{fig:roc_new_fea} shows, all variants of \textbf{genealogist} outperforms the feature \textit{No. callee} in terms of AUC value.
Furthermore, the algorithm \textbf{UpRelation} achieves the highest AUC value (0.977).


Similarly, to assess the filtration ability, we also calculate the $F_{score}$ for them, as shown in Figure~\ref{fig:fscore_new_fea}.
From the figure, our algorithm \textbf{UpRelation} has the highest $F_{score}$ 0.95 at the similarity threshold 0.79.

==> pretrain.tex <==

\todo{REASON for we adopt pretrain. and pretrain introduction.}

\noindent \textbf{Pretrained Model Selection.} Large pre-trained models such as BERT\todo{CITATION}, CodeBERT\todo{CITATION}, CodeT5 have dramatically improved the state-of-the-art methods in terms of natural language processing (NLP) and program language analysis (PLA) \todo{latest bert introduction paper}.
Pre-trained models aim to learn effective contextual representations from unlabeled code or text corpus.
Based on effective contextual representation, the methods in the downstream PLA tasks, such as code search, code generation, code completion et al., have made great progress compared with previous methods without applying pre-trained model.
In our work, we tend to integrate the pre-trained model for learning a better node embedding of AST.\todo{codebert models introduction and what we choose and why.}
CodeT5~\todo{citation} is used for node embedding of AST because it performs better than other pioneer models, such as CodeBERT~\todo{citation} and UnixCoder~\todo{citation}.
Tokenizing AST nodes by assigning distinct numbers starting at 1 to various types of AST nodes, is an essential step before training the CodeT5 model.
A tokenizer is trained and integrated in bert-like models to carry out the tokenization (of AST node) function.
Word splitting and word digitalization are the two sub-tasks that make up tokenization.
Word splitting divides a sentence into individual words and word digitalization converts a word to a number.
In our task, we treat an AST node as a word so we can just skip the word splitting step.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{pics/pretrained_model_codeT5.pdf}
    \caption{Overview of Pre-training Task.}
    \label{fig:pretrain_task}
\end{figure}

\subsection{AST Preprocessing and Model Pretraining.} 
\noindent\textbf{Serialization.}
Since CodeT5 accepts an array of numbers as input, we first serialize the AST into an AST node array (ANA) by preorder traversing the AST as shown in Figure~\ref{fig:pretrain_task}.
Every AST of binary function in the code base described in Section \ref{sec:codebase} undergoes AST serialization. 
Following that, we receive 267,580 ANAs for the CodeT5 training.

\noindent\textbf{Tokenization.}
We use all these ANAs to train our tokenizer. 
After training of tokenizer, the tokenizer generates a dictionary with 80 unique words that represent 80 different categories of AST nodes. 
Note that there are 43 different kinds of AST nodes introduced in our earlier work. In this work, we utilize the new version (7.7) of IDA Pro to acquire a more accurate and comprehensive AST following decompilation.
For example, we add `fmul' node to represent the float multiplication operation, which is not introduced in our previous work.

\noindent \textbf{Masking and MNP Task.}
The Bert-like model will often contain a number of pre-training tasks to direct the model as it learns semantics from corpus data.
For instance, CodeT5 has four pre-training tasks to learn knowledge from its program language data.
Unlike CodeT5's programming language data, the ASTs from our data base are serialized as ANAs, where each ANA corresponds to only one sentence in CodeT5's data.
There is just one pre-training task that is ideal for our ANA data, \textbf{masked node prediction} (MNP), because one ANA does not contain multiple sentences and other pre-training task (e.g., next sentence prediction) performs on multiple sentences.
Following ANA tokenization, the MNP task masks the node value in the ANA at random.
For example, \todo{${node1, node2, ... masked_i, ..., masked_j, node3.}$} is the input example of the MNP task.
MNP task predicts the node values of masked positions and compares the predicted node with groundtruth to tunes the model weights (by gradient descent algorithm~\todo{citation}).


\noindent \textbf{AST Embedding.}

\todo{Embedded AST definition here.}
